Counting Divisions of a $2\times n$ Rectangular Grid

Consider a $2\times n$ rectangular grid composed of $1\times 1$ squares. Cutting only along the edges between squares, how many ways are there to divide the board into $k$ pieces? Building off the work of Durham and Richmond, who found the closed-form solutions for the number of divisions into 2 and 3 pieces, we prove a recursive relationship that counts the number of divisions of the board into $k$ pieces. Using this recursion, we obtain closed-form solutions for the number of divisions for $k=4$ and $k=5$ using fitting techniques on data generated from the recursion. Furthermore, we show that the closed-form solution for any fixed $k$ must be a polynomial on $n$ with degree $2k-2$.

==> definitions.tex <==
We begin with the following definitions and remarks:
\begin{definition}
An $n\times m$ \textbf{board} is a rectangle consisting of $1\times 1$ \textbf{squares}. The board consists of $n$ squares vertically and $m$ squares horizontally. Two squares are \textbf{connected} if and only if they share an edge.
\end{definition}

\begin{definition}
A \textbf{cut} is an action that separates two connected squares along their shared edge.
\end{definition}

\begin{definition}
A \textbf{division} of a board into $k$ \textbf{pieces} is a sequence of cuts that result in the board being separated into $k$ connected components. See Figure~\ref{fig:exampledivision} for an example division of a $3\times 5$ board into 3 pieces.
\end{definition}

\begin{definition}
$d_k^m(n)$ denotes the number of divisions of an $n\times m$ board into $k$ pieces. For example, $d^3_3(5)$ is the number of divisions of a $3\times 5$ board into 3 pieces.
\end{definition}

\begin{definition}
$s_k^2(n)$ denotes the number of divisions of an $2\times n$ board into $k$ pieces where the two rightmost squares are separated by a cut along their shared edge. Likewise, $t_k^2(n)$ denotes the number of divisions of an $2\times n$ board into $k$ pieces where the two rightmost squares are not separated by a cut along their shared edge. Equivalently, this means the squares end up in the different pieces / the same piece, respectively.
\end{definition}


==> explaining_algorithm.tex <==
\section{Algorithm for Counting Divisions of $n\times m$ Board into $k$ Pieces} \label{sec:algorithm}

While $d_k^m(n)$ has directly proven explicit formulas for small values for $m$ and $k$, computational methods are much more useful to collect data about greater values. We used those data to fit polynomials that predict the number of divisions of the $2\times n$ board into more than two pieces; we prove those formulas satisfy the recursion of Theorem~\ref{drecursion} in the next section.

Our algorithm involves encoding the board as a graph, where the vertices represent the squares, and two vertices are adjacent if and only if their squares are connected in the board. A cut corresponds to removing an edge from the graph, and every valid division of the board corresponds to removing some set of edges from the graph to produce some number of connected components. The algorithm involves checking all possible combinations of edges to be removed, in other words, it iterates through the power set of the edge set of the graph, and finds the number of connected components for each graph after the edge removal. We implemented our algorithm in Python using Networkx [3] and Numpy [4].

However, not every sequence of cuts results in a valid division. For a division to be valid, any two squares that are separated by a cut must end up in different pieces of the division. In the algorithm, this means that if two vertices are adjacent before the edge removal and are not adjacent after the edge removal, the two vertices must not be in the same connected component of the resulting graph.

Using this check for validity, the following algorithm returns the number of divisions of an $n\times m$ board into $1$ through $mn$ pieces. While the algorithm is computationally expensive, it is exhaustive. Therefore no divisions are missed by the algorithm and the divisions into all numbers of pieces are returned by the algorithm at once.


==> formula_proofs.tex <==
\begin{lemma}
$\displaystyle s_3^2(n)=\frac{4}{3}n^3-3n^2+\frac{8}{3}n-1$
\label{s3_closed}
\end{lemma}
\begin{proof}
For the base case, there are 0 divisions of the $2\times 1$ board into 3 pieces, meaning there must be 0 divisions where the rightmost pieces separate, so $s_3^2(1)=0$. The closed form solution has a root at $n=1$, so this satisfies the base case. For the inductive assumption, assume the above closed form solution holds for $n$. Then, from Theorem~\ref{s_recursion}, Theorem~\ref{the:twopieces}, and Remark~\ref{re:onedivision}:
\begin{align*}
s_3^2(n+1)&=d_1^2(n)+2d_2^2(n)+\frac{4}{3}n^3-3n^2+\frac{8}{3}n-1\\
&=(1)+2n(2n-1)+\frac{4}{3}n^3-3n^2+\frac{8}{3}n-1\\
&=\frac{4}{3}n^3+n^2+\frac{2}{3}n\\
&=\frac{4}{3}(n+1)^3-3(n+1)^2+\frac{8}{3}(n+1)-1
\end{align*}
\end{proof}
With this result, a closed form solution for $d_3^2(n)$ can be found.
\begin{theorem}[Durham]
$\displaystyle d_3^2(n)=\frac{2}{3}n^4-\frac{4}{3}n^3+\frac{11}{6}n^2-\frac{13}{6}n+1$
\label{d3_closed}
\end{theorem}
\begin{proof}
For the base case, there are 0 divisions of the $2\times 1$ board into 3 pieces, so $d_3^2(1)=0$, and the closed form solution has a root at $n=1$, which satisfies the base case. For the inductive assumption, assume the above closed form solution holds for $n$. Then substituting using Lemma~\ref{s3_closed}:
\begin{align*}
d_3^2(n+1)&=d_1^2(n)+3d_2^2(n)+d_3^2(n)+2s_3^2(n)\\
&= (1)+3n(2n-1)+\frac{2}{3}n^4-\frac{4}{3}n^3+\frac{11}{6}n^2-\frac{13}{6}n+1\\
&\quad+2\left(\frac{4}{3}n^3-3n^2+\frac{8}{3}n-1\right)\\
&= \frac{2}{3}n^4+\frac{4}{3}n^3+\frac{11}{6}n^2+\frac{1}{6}n\\
&= \frac{2}{3}(n+1)^4-\frac{4}{3}(n+1)^3+\frac{11}{6}(n+1)^2-\frac{13}{6}(n+1)+1
\end{align*}
\end{proof}
Again using the recursive relations from the third section, we can find an explicit formula for $d_4^2(n)$. First, a closed form of $s_4^2(n)$ is found.
\begin{lemma}
$\displaystyle s_4^2(n)=\frac{4}{15}n^5-\frac{4}{3}n^4+\frac{11}{3}n^3-\frac{37}{6}n^2+\frac{167}{30}n-2$
\label{s4_closed}
\end{lemma}
\begin{proof}
The same argument applies for the base case as in the divisions into three pieces, so $s_4^2(1)=0$. For the inductive assumption, assume the above closed form solution holds for $n$. Then, from Theorem~\ref{s_recursion}:
\begin{align*}
s_4^2(n+1)&=d_2^2(n)+2d_3^2(n)+\frac{4}{15}n^5-\frac{4}{3}n^4+\frac{11}{3}n^3-\frac{37}{6}n^2+\frac{167}{30}n-2\\
&=n(2n-1)+2\left(\frac{2}{3}n^4-\frac{4}{3}n^3+\frac{11}{6}n^2-\frac{13}{6}n+1 \right)\\
&\quad+\frac{4}{15}n^5-\frac{4}{3}n^4+\frac{11}{3}n^3-\frac{37}{6}n^2+\frac{167}{30}n-2\\
&=\frac{4}{15}n^5+n^3-\frac{1}{2}n^2+\frac{7}{30}n\\
&=\frac{4}{15}(n+1)^5-\frac{4}{3}(n+1)^4+\frac{11}{3}(n+1)^3\\
&\quad-\frac{37}{6}(n+1)^2+\frac{167}{30}(n+1)-2
\end{align*}
\end{proof}
With this result, a closed form solution for $d_4^2(n)$ can be found.
\begin{theorem}
$\displaystyle d_4^2(n)=\frac{4}{45}n^6-\frac{2}{5}n^5+\frac{25}{18}n^4-\frac{7}{2}n^3+\frac{226}{45}n^2-\frac{18}{5}n+1$
\label{d4_closed}
\end{theorem}
\begin{proof}
The same argument applies for the base case as in the divisions into three pieces, so $d_4^2(1)=0$. For the inductive assumption, assume the above closed form solution holds for $n$. Then substituting using Lemma~\ref{s4_closed}:
\begin{align*}
d_4^2(n+1)&=d_2^2(n)+3d_3^2(n)+d_4^2(n)+2s_4^2(n)\\
&= n(2n-1)+3\left(\frac{2}{3}n^4-\frac{4}{3}n^3+\frac{11}{6}n^2-\frac{13}{6}n+1\right)\\
&\quad+\frac{4}{45}n^6-\frac{2}{5}n^5+\frac{25}{18}n^4-\frac{7}{2}n^3+\frac{226}{45}n^2-\frac{18}{5}n+1\\
&\quad+2\left(\frac{4}{15}n^5-\frac{4}{3}n^4+\frac{11}{3}n^3-\frac{37}{6}n^2+\frac{167}{30}n-2\right)\\
&= \frac{4}{45}n^6+\frac{2}{15}n^5+\frac{13}{18}n^4-\frac{1}{6}n^3+\frac{17}{90}n^2+\frac{1}{30}n\\
&= \frac{4}{45}(n+1)^6-\frac{2}{5}(n+1)^5+\frac{25}{18}(n+1)^4\\
&\quad-\frac{7}{2}(n+1)^3+\frac{226}{45}(n+1)^2-\frac{18}{5}(n+1)+1
\end{align*}
\end{proof}
\begin{lemma}
$$ s_5^2(n)=\frac{25}{1008}n^7-\frac{37}{180}n^6+\frac{71}{72}n^5-\frac{107}{36}n^4+\frac{751}{144}n^3-\frac{217}{45}n^2+\frac{149}{84}n$$
\label{lem:s_5}
\end{lemma}
\begin{theorem}
$\displaystyle d_5^2(n)=\frac{2}{315}n^8+\frac{2}{15}n^6-\frac{1}{5}n^5+\frac{49}{120}n^4-\frac{7}{12}n^3+\frac{1139}{2520}n^2-\frac{13}{60}n$
\label{the:d_5}
\end{theorem}
\begin{proof}
For proofs of Lemma~\ref{lem:s_5} and Theorem~\ref{the:d_5}, see supplementary material.
\end{proof}

==> old_degree_proofs.tex <==
\begin{lemma}
Let $p(n)$ be a polynomial with a positive leading coefficient. $p(n)$ is of degree $d$ if and only if for all $C,c\in\mathbb{R}^+$, there exists an $N\in\mathbb{R}^+$, that depends on $C$ and $c$, such that for all $n>N$, $Cn^{d-1}<p(n)<cn^{d+1}$.
\label{lem:bound_polynomail}
\end{lemma}
\begin{proof}
Suppose that for all $C,c>0$, there exists an $N$, that depends on $C$ and $c$, such that for all $n>N$, $Cn^{d-1}<p(n)<cn^{d+1}$. Let $n\neq0$, and divide throughout by $n^{d-1}$. Thus, for all $n>N$, $\displaystyle C<\frac{p(n)}{n^{d-1}}<cn^2$. The only function that satisfies this string of inequalities for all values of $C$ and $c$ is for $\frac{p(n)}{n^{d-1}}$ to be a linear function. Thus, $p(n)$ is of degree $d$.

Now suppose $p(n)$ is of degree $d$. Then $p(n)=An^d+\mathcal{O}(d-1)$, where $A>0$ and $\mathcal{O}(d-1)$ are the lower-order terms. Consider $P(n)=p(n)-Cn^{d-1}$. This polynomial determines whether or not $p(n)>Cn^{d-1}$, as $P(n)>0$ when $p(n)>Cn^{d-1}$. To show that there exists an $N$ such that $P(n)>0$ for all $n>N$, it suffices to show that there exists an input $N_1$ such that $P(n)>0$ and $P'(n)>0$ for all $n>N_1$. Because $A>0$ and the degree of $p(n)$ is greater than $d-1$, $P(n)\to\infty$ as $n\to\infty$.

Now consider the derivative of $P(n)$. $P'(n)=dAn^{d-1}+\mathcal{O}(d-2)- C(d-1)n^{d-2}$, and because $dA>0$, it means that $P'(n)\to\infty$ as $n\to\infty$, so the function is strictly increasing after some point.

Therefore, there must be some number $N_1$ such that $P(n)>0$ and $P'(n)>0$ for all $n>N_1$, meaning $Cn^{d-1}<p(n)$ for all $n>N_1$.

Now consider $Q(n)=p(n)-cn^{d+1}$.  Again, to show there exists an $N$ such that $Q(n)<0$ for all $n>N$, it suffices to show that there exists an input $N_2$ such that $Q(N_2)<0$ and that $Q'(N_2)<0$ for all $n>N_2$. Because $c>0$ and the degree of $p(n)$ is less than $d+1$, $Q(n)\to-\infty$ as $n\to\infty$.

Now consider the derivative of $Q(n)$. $Q'(n)=dAn^{d-1}+\mathcal{O}(d-2)- c(d+1)n^{d}$, and because $c(d+1)>0$, it means that $Q'(n)\to-\infty$ as $n\to\infty$, so the function is strictly decreasing after some point.

Therefore, there must be some number $N_2$ such that $Q(n)<0$ and $Q'(n)<0$ for all $n>N_2$, meaning $p(n)<cn^{d+1}$ for all $n>N_2$. Choose $N=\max\{N_1,N_2\}$. Thus for all $n>N$, $Cn^{d-1}<p(n)<cn^{d+1}$.
\end{proof}
We now prove a lemma about how the degree of a polynomial $p(n)$ is equal to a different polynomial that is constructed using $p(n)$ 

\begin{lemma}
Let $p(n)$ be a polynomial. Then $p(n)$ and $n(p(n+1)-p(n))$ are the same degree.
\label{lem:same_degree}
\end{lemma}
\begin{proof}
Suppose $p(n)$ is of degree $d$. Then $p(n)=An^d+Bn^{d-1}+\mathcal{O}(d-2)$ and $p(n+1)=A(n+1)^d+B(n+1)^{d-1}+\mathcal{O}(d-2)$. Expanding using the binomial theorem, 
\begin{equation*}
p(n+1)=An^d+A(d-1)n^{d-1}+Bn^{d-1}+\mathcal{O}(d-2)
\end{equation*}
Subtracting,
\begin{align*}
p(n+1)-p(n)&=An^d+A(d-1)n^{d-1}+Bn^{d-1}+\mathcal{O}(d-2)\\
&\quad\quad\quad-An^d-Bn^{d-1}-\mathcal{O}(d-2)\\
&=A(d-1)n^{d-1}+\mathcal{O}(d-2)
\end{align*}
Multiplying through by $n$:
\begin{equation*}
n(p(n+1)-p(n))=A(d-1)n^{d}+\mathcal{O}(d-1)
\end{equation*}
Which is of degree $d$.
\end{proof}
We now have all the information to prove the degree of the division-counting polynomial for a given $k$.

==> s5d5_proofs.tex <==
\begin{lemma}
$$s_5^2(n)=\frac{25}{1008}n^7-\frac{37}{180}n^6+\frac{71}{72}n^5-\frac{107}{36}n^4+\frac{751}{144}n^3-\frac{217}{45}n^2+\frac{149}{84}n$$
\label{lem:s_5}
\end{lemma}
\begin{proof}
\begin{align*}
    s_5^2(n+1)&=d_3^2(n)+2d_4^2(n)\\
    &\quad+\frac{25}{1008}n^7-\frac{37}{180}n^6+\frac{71}{72}n^5-\frac{107}{36}n^4+\frac{751}{144}n^3-\frac{217}{45}n^2+\frac{149}{84}n\\
    &=\frac{2}{3}n^4-\frac{4}{3}n^3+\frac{11}{6}n^2-\frac{13}{6}n+1\\
    &\quad+2\left(\frac{4}{45}n^6-\frac{2}{5}n^5+\frac{25}{18}n^4-\frac{7}{2}n^3+\frac{226}{45}n^2-\frac{18}{5}n+1\right)\\
    &\quad+\frac{25}{1008}n^7-\frac{37}{180}n^6+\frac{71}{72}n^5-\frac{107}{36}n^4+\frac{751}{144}n^3-\frac{217}{45}n^2+\frac{149}{84}n\\
    &=\frac{25}{1008}(n+1)^7-\frac{37}{180}(n+1)^6+\frac{71}{72}(n+1)^5-\frac{107}{36}(n+1)^4\\
    &\quad+\frac{751}{144}(n+1)^3-\frac{217}{45}(n+1)^2+\frac{149}{84}(n+1)
\end{align*}

\end{proof}

==> symmetry.tex <==
\section{Symmetry of Divisions}\label{sec:sym}

Consider the two divisions shown in Figure~\ref{fig:symmetry}. One could reasonably argue that these two divisions are the same, as one can be obtained from the other by simply reflecting the board along a horizontal or vertical axis. This raises the question: is there a way to count the divisions that are the same under isometric transformations of the board, that is, rotations and reflections?

To answer this question, we introduce the following definition:

\begin{definition}
Two divisions are \textbf{equivalent up to isometry} if and only if one division can be mapped onto the other by rotating or reflecting the board. The number of divisions up to isometry is denoted as $i_2^2(n)$
\end{definition}

Equivalence up to isometry forms an equivalence relation over the set of divisions of the board, therefore, there is a set of equivalence classes under this equivalence relation. Each division in an equivalence class can be obtained from the others by rotating and reflecting the overall board. Therefore, each equivalence class is an orbit of the divisions under the group actions of rotation and reflection. In this case, these actions correspond to the dihedral group of order 4, $\mathcal{D}_2$. This calls to mind Burnside's Lemma [5]:
\begin{lemma}[Burnside's Lemma]
Let $X$ be a set and $G$ be a group acting on the set. If $X^g$ is the set of elements in $X$ that are fixed by each $g\in G$, then the number of orbits $|X/G|$ of $X$ when acted upon by $G$ is
\begin{equation*}
|X/G|=\frac{1}{|G|}\sum_{g\in G}|X^g|
\end{equation*}
\label{burnside}
\end{lemma}
\begin{figure}
    \centering
    \includegraphics[width=9cm]{symmetry.eps}
    \caption{Reflecting the board along a horizontal or vertical axis maps one division onto the other.}
    \label{fig:symmetry}
\end{figure}
Before moving on to counting the divisions up to isometry, a couple additional lemmas will be proven to facilitate the arguments.
\begin{lemma}
For a $2\times n$ board being divided into 2 pieces, there are at most 2 vertical cuts.
\end{lemma}
\begin{proof}
Consider a division consisting of 3 or more vertical cuts. Either three cuts are on the same row, or two are on one row and one is on the other. If three are on the same row, then one cut must be between the other two. The outer two cuts will form a division consisting of a rectangular piece and the remainder of the board. The third vertical cut will divide this rectangular piece into two pieces, giving three in total. If two are on one row and one is on the other, there are three cases: (i) one cut is between the other two, and the outer cuts are on the same row, (ii) one cut is between the other two, and the outer cuts are on different rows, (iii) the single cut in one row aligns with one of the two cuts in the other row.
\\ \\
For case (i), the outer cuts will form a division consisting of a rectangular piece and the remainder of the board. The third cut will divide the remainder of the board, giving three total. For case (ii), the outer cuts will form a division consisting of an L-shaped piece and the remainder of the board. The third cut will divide this L-shaped piece into two pieces, giving three in total. For case (iii), the two cuts on the same row will form a division consisting of a rectangle and the remainder of the board. The third cut will divide the remainder of the board, giving three in total.
\end{proof}
\begin{lemma}
Any division fixed by rotation must consist of isometrically identical pieces.
\label{identical_rotation}
\end{lemma}
\begin{proof}
Consider a division consisting of non-identical pieces. In order for a rotation to fix a division, when rotated, each piece must map exactly to where the other piece was previously. If the pieces are shaped differently, then neither piece will fit into where the other piece was previously, meaning the division cannot be fixed by rotation. This means a division consisting of non-identical pieces is not fixed by rotation, and the contrapositive must also be true.
\end{proof}
\begin{lemma}
Any division fixed by reflection must map vertical cuts to vertical cuts.
\label{cuts_reflection}
\end{lemma}
\begin{proof}
Suppose there is a reflection that does not map vertical cuts to vertical cuts. Then, after the reflection, the division will be different, as the vertical cuts are not in the same place as before. This means that any reflection that does not map vertical cuts to vertical cuts cannot fix any division, and the contrapositive must also be true.
\end{proof}
\begin{lemma}
Let $g\in \mathcal{D}_2$ not be the identity action. Then for each $x\in X^g$, there must be 0 or 2 vertical cuts. If there are 2, they must be the same distance from the vertical axis of reflection.
\label{lem:not_identity}
\end{lemma}
\begin{proof}
A division consisting of only 1 vertical cut cannot be fixed by any non-identity group action. This is because a single vertical cut corresponds to a division that results in a corner being removed from the main board. The non-rectangular remainder of the board is cannot be fixed by any rotation or reflection, so the division as a whole cannot be fixed by any group action.
\\ \\
Consider a division consisting of 2 vertical cuts. Suppose that the two cuts are not the same distance from the vertical axis of reflection, which means they cannot be identical. Then the pieces cannot be fixed by any symmetry in $\mathcal{D}_2$. By Lemma~\ref{identical_rotation}, they cannot be fixed by the rotation because they are not identical. By Lemma~\ref{cuts_reflection}, they cannot be fixed by any reflection because any such reflection cannot map vertical cuts to vertical cuts, as they will not ``align" with one another. Therefore any division where the vertical cuts are not the same distance from the vertical axis of reflection cannot by fixed by any non-identity group action, and the contrapositive must also be true.
\end{proof}
We now have the capability to prove the following theorem:
\begin{theorem}
The number of divisions up to isometry for the $2\times n$ board into two pieces is
$$i_2^2(n)=\frac{1}{2}n(n+1)$$.
\label{the:symmetry}
\end{theorem}
\begin{proof}
Let $D_2^2(n)$ be the set of divisions of the $2\times n$ board into 2 pieces. The number of divisions up to isometry is equal to the number of orbits of $D_2^2(n)$ under the elements of $\mathcal{D}_2$. These are counted using Burnside's Lemma:
\begin{equation*}
   i^2_2(n)=\frac{1}{|\mathcal{D}_2|}\sum_{g\in \mathcal{D}_2}|D_2^2(n)^g|
\end{equation*}
Recall that $\mathcal{D}_2=\{e,\rho,\mu_H,\mu_V\}$, where $e$ is the identity, $\rho$ is a rotation by $180^\circ$, $\mu_H$ is a horizontal reflection, and $\mu_V$ is a vertical reflection. 

Clearly, all elements of $D_2^2(n)$ are fixed by $e$, so $|D_2^2(n)^e|=d_2^2(n)=2n^2-n$.

For $\rho$, recall from Lemma~\ref{identical_rotation} that any division fixed by rotation must consist of identical pieces, and from Lemma~\ref{lem:not_identity} that the division must consist of 0 or 2 vertical cuts. If there are 0, then the board must be cut completely in half along the horizontal middle, which corresponds to 1 division. 

If there are 2, then they must be the same distance from the vertical axis of reflection. To produce identical pieces, the two vertical cuts must be on opposite sides both the horizontal and vertical axes of reflection, corresponding to a division that creates two identical L-shaped pieces. There are $n-1$ ways to choose where to place the cut above the horizontal axis, which fixes the location of the second cut. This corresponds to $n-1$ divisions. Therefore, there are $n$ divisions fixed by rotation.

For $\mu_H$, recall from Lemma~\ref{cuts_reflection} that any division fixed by reflection must consist of identical pieces, and from Lemma~\ref{lem:not_identity} that the division must consist of 0 or 2 vertical cuts. If there are 0, then the board must be cut completely in half along the horizontal middle, which corresponds to 1 division. 

If there are 2, then they must be the same distance from the vertical axis of reflection. To map vertical cuts to vertical cuts, the two vertical cuts must be on opposite sides both the horizontal axis of reflection, but on the same side of the vertical axis of reflection, corresponding to a division that cuts the board along a vertical cut of length 2. There are $n-1$ ways to choose where to place the cut above the horizontal axis, which fixes the location of the second cut. This corresponds to $n-1$ divisions. Therefore, there are $n$ divisions fixed by horizontal reflection.

For $\mu_V$, recall from Lemma~\ref{cuts_reflection} that any division fixed by reflection must consist of identical pieces, and from Lemma~\ref{lem:not_identity} that the division must consist of 0 or 2 vertical cuts. If there are 0, then the board must be cut completely in half along the horizontal middle, which corresponds to 1 division. 

If there are 2, then they must be the same distance from the vertical axis of reflection. To map vertical cuts to vertical cuts, the two vertical cuts must be on the same side of horizontal axis of reflection, but on opposite sides of the vertical axis of reflection, corresponding to a division that cuts a rectangle out of one side of the board, leaving a cup-shaped piece on the other side. There are $n-1$ ways to choose where to place the first cut, which fixes the location of the second cut. This corresponds to $n-1$ divisions. Therefore, there are $n$ divisions fixed by vertical reflection.

Putting everything together:
\begin{equation*}
    i_2^2(n)=\frac{1}{4}(2n^2-n+n+n+n)=\frac{1}{4}(2n^2+2n)=\frac{1}{2}n(n+1)
\end{equation*}
\end{proof}

==> table.tex <==
\section{Table of Values}

\begin{table}[h]
    \centering
    \begin{tabular}{l|ccccc}
$n$\textbackslash $k$&1&2&3&4&5\\\hline
1&1&1&0&0&0\\
2&1&6&4&1&0\\
3&1&15&29&21&7\\
4&1&28&107&153&111\\
5&1&45&286&678&831\\
6&1&66&630&2241&4131\\
7&1&91&1219&6091&15748\\
8&1&120&2149&14385&49728\\
9&1&153&3532&30556&136322\\
10&1&190&5496&59745&334650\\
11&1&231&8185&109297&751797\\
12&1&276&11759&189321&1570261\\
13&1&325&16394&313314&3085929\\
14&1&378&22282&498849&5759013\\
15&1&435&29631&768327&10280634\\
16&1&496&38665&1149793&17657998\\
17&1&561&49624&1677816&29321364\\
18&1&630&62764&2394433&47256260\\
19&1&703&78357&3350157&74164659\\
20&1&780&96691&4605049&113659083\\\hline
$n$\textbackslash $k$&6&7&8&9&10\\\hline
1&0&0&0&0&0\\
2&0&0&0&0&0\\
3&1&0&0&0&0\\
4&45&10&1&0&0\\
5&603&274&78&13&1\\
6&4596&3334&1635&545&120\\
7&24732&25747&18667&9668&3600\\
8&104575&146831&145602&105508&56931\\
9&369826&671848&868084&829399&600723\\
10&1138712&2596968&4227342&5121823&4751906\\
11&3138171&8779022&17557890&26233173&30193383\\
12&7896713&26600748&64099355&115621525&161241434\\
13&18416453&73572842&210256970&450245602&747044478\\
14&40266876&188347198&630047025&1579913534&3073562178\\
15&83292430&451183577&1747134845&5071899551&11430370077\\
16&164186075&1020203769&4529679900&15074867903&38959972033\\
17&310252468&2193013248&11071498344&41885398146&123062891994\\
18&564768560&4507745568&25686998844&109653320338&363498052540\\
19&994447045&8903613660&56893770324&272254496222&1011537069434\\
20&1699620357&16969012366&120878343957&644635341150&2668573664500\\
    \end{tabular}
    \label{tab:my_label}
\end{table}

==> two_pieces.tex <==
\section{Closed Form Solution for Counting Divisions into Two Pieces} \label{sec:twopieces}
Durham and Richmond previously showed that the number of divisions of the $2\times n$ board into two pieces is given by $2n^2-n$. Wagon~\cite{wagon} provided an alternative visual proof to their result, we offer yet another alternative proof. Our argument makes use of induction and recursion, and these arguments will be utilized in a similar manner in the following sections. A key insight to our argument is that the divisions of a $2\times n$ board are embedded within the divisions of a $2\times (n+1)$ board, and the divisions of this ``sub-board" (consisting of all but the rightmost column) correspond in a predictable manner with the divisions of the overall board.
\begin{theorem}[Durham]
\label{the:twopieces}
The number of divisions of a $2\times n$ board into two pieces is $d^2_2(n)=n(2n-1)$.
\end{theorem}
\begin{proof}

Our proof is by induction on $n$.

By Remark~\ref{re:onedivision}, $d^2_2(1)=1=(1)(2(1)-1)$.

For the induction, assume for a positive integer $j$ that $d_2^2(j)=j(2j-1)$. Each division of the $2\times j$ sub-board has some number of corresponding divisions in the $2\times (j+1)$ board. Note that the sub-board's division may be into only one piece. Color the rightmost vertically-connected squares of the $2\times(j+1)$ board blue and the rightmost vertically-connected squares of the $2\times j$ sub-board green (see Figure~\ref{fig:greenblue}). To obtain a division into two pieces on the $2\times(j+1)$ board, there are two cases to consider. First, there's the case where the $2\times j$ sub-board is divided into only one piece. In this case, there are three ways to obtain a division of the $2\times (j+1)$ board into two pieces. Two divisions can be obtained by cutting off one of the blue squares and attaching the other to the $2\times j$ sub-board, and one division is obtained by cutting off both blue squares into their own piece (see Figure~\ref{fig:greentogether}). 
\begin{figure}
\centering
\includegraphics[width=5cm]{twocolor.eps}
\caption{Coloring argument that is used in the proof of Theorem~\ref{the:twopieces}.}
\label{fig:greenblue}
\end{figure}

The remaining divisions can be obtained by dividing the $2\times j$ sub-board into two pieces and adding the blue squares onto them. Recall from Lemma~\ref{lem:separation} that the number of divisions of the $2\times j$ sub-board is partitioned by whether or not the green squares separate. Furthermore, for each division, there will be some number of ways to add the blue squares to obtain a division of the $2\times (j+1)$ board. Therefore, we can write:
\begin{equation}
\label{eq:divisionsincomplete}
d_2^2(j+1)=3+At_2^2(j)+Bs_2^2(j)
\end{equation}
For some positive integers $A,B$. To find $A$, note that when the green squares do not separate, the blue squares must remain connected and attach to the green squares, or else the board will be divided into more than two pieces. Therefore, for each division of the $2\times j$ sub-board where the green squares do not separate, there is one corresponding division in the $2\times (j+1)$ board. Thus, $A=1$

\begin{figure}
\centering
\includegraphics[width=12 cm]{sep.eps}
\caption{The three ways for the blue squares to be added to the board when the $2\times j$ sub-board remains fully intact. The case on the left accounts for two ways, depending on which blue square becomes its own piece.}
\label{fig:greentogether}
\end{figure}

When the green squares do separate, there are three possible sub-cases: i) both blue squares attach to the top green square, ii) both blue squares attach to the bottom green square, or iii) the blue squares separate and attach one to each green square (see Figure~\ref{fig:addgreenseparate}). Therefore, for each division of the $2\times j$ board where the green squares do separate, there are 3 corresponding divisions in the $2\times (j+1)$ board, thus $B=3$.

\begin{figure}
\centering
\includegraphics[width=12cm]{threesep.eps}
\caption{The three ways to add the blue squares to a division of the $2\times j$ sub-board where the green squares separate.}
\label{fig:addgreenseparate}
\end{figure}



Rewriting Equation~\ref{eq:divisionsincomplete} using Lemma~\ref{lem:separation}:
\begin{equation}
d_2^2(j+1)=3+t_2^2(j)+3s_2^2(j)=3+2s_2^2(j)+d_2^2(j)
\label{eq:divisionscomplete}
\end{equation}

To count $s_2^2(j)$, note that the only divisions of the $2\times j$ sub-board that cause the green squares to separate are the division that divides the board along the horizontal middle and the divisions that remove only the corner of the board. To remove only a corner of the board, place a vertical cut along any of the $j-1$ vertical edges that are contained in the interior of the board (ie, those edges that are not on the outer boundary). Then, make a horizontal cut along the horizontal middle of the board in the direction of the corner to be removed (See Figure~\ref{fig:greenseparate}). Thus, there are $j-1$ ways to remove one corner from the board, and because there are two corners being considered, the total number of divisions that separate the green squares is
\begin{equation*}
s_2^2(j)=2(j-1)+1=2j-1
\end{equation*}

Substituting this into Equation~\ref{eq:divisionscomplete}, and using the inductive assumption:
\begin{equation*}
d_2^2(j+1)=3+2(2j-1)+j(2j-1)=2j^2+3j+1=(j+1)(2(j+1)-1)
\end{equation*}
Which completes the induction.
\end{proof}
\begin{figure}
\centering
\includegraphics[width=4cm]{endoff.eps}
\caption{Each vertical red line is a possible edge to place a vertical cut that, when paired with the horizontal cut to the right edge of the board, removes the upper right corner of the board and results in the green squares becoming separated.}
\label{fig:greenseparate}
\end{figure}
The ``adding squares" approach from this section forms the core of our arguments for the next section. This strategy highlights how the number of divisions depends on the number of divisions of the board into a smaller number of pieces. In addition, there is a further dependence on \textit{how} the divisions are structured, particularly by whether or not the rightmost squares end up in separate pieces.

